Arabidopsis roots segmentation based on morphological operations and CRFs

Arabidopsis thaliana is a plant species widely utilized by scientists to estimate the impact of genetic differences in root morphological features. For this purpose, images of this plant after genetic modifications are taken to study differences in the root architecture. This task requires manual segmentations of radicular structures, although this is a particularly tedious and time-consuming labor. In this work, we present an unsupervised method for Arabidopsis thaliana root segmentation based on morphological operations and fully-connected Conditional Random Fields. Although other approaches have been proposed to this purpose, all of them are based on more complex and expensive imaging modalities. Our results prove that our method can be easily applied over images taken using conventional scanners, with a minor user intervention. A first data set, our results and a fully open source implementation are available online.

==> stateoftheart.tex <==
\section{State of the art}
\label{sec:stateoftheart}

Several attempts have been made in the last 20 years to solve the problem of segmenting the vascular tree on fundus images, but none of the resulted algorithms have yet proved to be accurate enough to be assumed as a standard by the medical community \cite{fraz2012blood}. In general, these approaches can be classified into two categories, supervised and unsupervised. Supervised methods require a set of labeled training samples to learn a model. These samples are typically composed of pixels features and their known annotations. Unsupervised methods involve different systems that are able to detect the retinal vasculature without requiring any training data. 

Most of the effort in supervised segmentation involves finding additional features to better describe vessel pixels, or better classifiers to perform the vessel classification task. In \cite{niemeijer2004comparative}, a $k$-nearest neighbors classifier fed with first order derivatives of Gaussians and green bands on original color fundus images is compared with respect to other unsupervised methods. The pixel classification approach proves to achieve better performance than other unsupervised methods, although it remains to be lower than the achieved by a second human observer. The same classification method is considered in \cite{staal2004ridge}, but using a different set of features. Authors utilize ridge detection to form line elements and partition the image into patches belonging to each line element. Pixel features are then generated based on this representation, and a feature selection scheme is used to choose those which provide the best class separability. Soares \textit{et al.} \cite{soares2006retinal} combine a Bayesian classifier with responses to the Gabor wavelet transform taken at multiple scales to yield a fast classification. Marin \textit{et al.} \cite{marin2011new} train a neural network with gray level and moment invariants based features extracted from a subset of hand-picked image pixels. Ricci and Perfetti \cite{ricci2007retinal} demonstrate that support vector machines combined with a line detector based feature outperforms thresholding in terms of accuracy and area under the receiver operating characteristic curve. An ensemble system of bagged and boosted decision trees, combined with features based on the orientation analysis of gradient vector field, morphological transformations, line strength measures and Gabor filter responses is proposed in \cite{fraz2012ensemble}. In \cite{you2011segmentation}, authors propose a semi-supervised self-training method to extract the major structures of vessels. More recently, Roychowdury \textit{et al.} \cite{roychowdhury2014blood} utilize a Gaussian Mixture Model classifier to refine an initial segmentation obtained by a combination of high-pass filtering and a vessel enhancement technique based of morphological reconstruction. Eight features extracted from pixel neighborhood and first and second-order gradient images are used to feed the classifier.

Current literature abounds of unsupervised approaches, mostly based on thresholding \cite{chaudhuri1989detection, hoover2000locating, zana2001segmentation, jiang2003adaptive, zhang2009detection, zhang2010retinal, ng2010maximum, miri2011retinal, fraz2012approach, bankhead2012fast, fathi2013automatic}, vessel tracking \cite{delibasis2010automatic, vlachos2010multi} or region-oriented approaches such as region growing \cite{mendonca2006segmentation, martinez2007segmentation, palomera2010parallel} or snakes \cite{espona2007snake, espona2008retinal}. 

Existing works based on thresholding used to be focused on the development of new techniques for vessel enhancement. Mathematical morphology has emerged as a proficient technique in this sense. Zana and Klein \cite{zana2001segmentation}, for instance, introduce a combination of different morphological operations that proves to be effective in the characterization of blood vessels. Authors obtain the final segmentation by thresholding the resulting enhanced image. A different techniques is proposed in \cite{chaudhuri1989detection}, where it is shown that the gray level profile of the cross section of a retinal blood vessel can be approximated by a Gaussian shaped curve. Following this prior, authors suggest to enhance vessels by matching a Gaussian profile at different orientations, and taking the maximum response to the filter at different scales. This technique is known as matched filter, as is combined with thresholding approaches in several works. In \cite{hoover2000locating}, for instance, authors recover the vessel network from matched filter responses by iteratively collecting its pieces at different thresholds. Since matched filters have difficulties to characterize narrow vessels and also produce false detections in the presence of pathologies, Zhang \textit{et al.} suggest to include an additional filter based on the first order derivative of the Gaussian \cite{zhang2010retinal}. This new version of original matched filter is analyzed in \cite{fraz2012approach} to extract vessel centerlines at different orientations. These structures are then processed with morphological operators to reconstruct vessels. In \cite{ng2010maximum}, second order derivative of Gaussians are applied at several scales, and the filter outputs are used to infer the presence of vessels and their properties. By taking into account this information, a maximum likelihood model based approach is applied to recover probability maps, which are afterwards thresholded to obtain the segmentations. Morphological operations are also considered in \cite{miri2011retinal}, where authors utilize them to construct ridges from images enhanced with a modification of discrete curvelet transform coefficient. The final segmentation is obtained by thresholding the resulting image. Responses to different types of wavelets--such as the isotropic undecimated wavelet transform \cite{bankhead2012fast} or the complex continuous wavelet transform \cite{fathi2013automatic}--have been also proposed to improve blood vessels discrimination before applying thresholding. The approach introduced in \cite{zhang2009detection} uses the nonlinear orthogonal projection to capture the features of vessel networks, and derives a novel local adaptive thresholding algorithm for vessel detection. A different version of adaptive thresholding method was proposed in \cite{jiang2003adaptive} before. Instead of being evaluated over a vessel enhanced image, in this work authors only consider the green band of the original color image.

Vessel tracking algorithms work at the level of a single vessel rather than the entire vasculature. Given two points, these type of methods first localize the centerline of the vessel by trying to find the path which better matches a given profile model. In this sense, Delibasis \textit{et al.} utilizes a parametric model of a vessel composed of a stripe which exploits geometric properties to define the parameters. A match metric is defined also to quantify the similarity between the model and the given image. Other vessel tracking approach is explained in \cite{vlachos2010multi}

Snakes, also known as deformable contours, can be interpreted 

%region growing \cite{mendonca2006segmentation, martinez2007segmentation, palomera2010parallel} 
%
%snakes \cite{espona2007snake, espona2008retinal}

%\cite{}
